Disentangled Person Image Generation

Generating novel, yet realistic, images of persons is a challenging task due to the complex interplay between the different image factors, such as the foreground, background and pose information. In this work, we aim at generating such images based on a novel, two-stage reconstruction pipeline that learns a disentangled representation of the aforementioned image factors and generates novel person images at the same time. First, a multi-branched reconstruction network is proposed to disentangle and encode the three factors into embedding features, which are then combined to re-compose the input image itself. Second, three corresponding mapping functions are learned in an adversarial manner in order to map Gaussian noise to the learned embedding feature space, for each factor respectively. Using the proposed framework, we can manipulate the foreground, background and pose of the input image, and also sample new embedding features to generate such targeted manipulations, that provide more control over the generation process. Experiments on Market-1501 and Deepfashion datasets show that our model does not only generate realistic person images with new foregrounds, backgrounds and poses, but also manipulates the generated factors and interpolates the in-between states. Another set of experiments on Market-1501 shows that our model can also be beneficial for the person re-identification task.

==> 10-supp_sampling.tex <==
\section{Image sampling results}
\label{sec:supp_sampling}

We also give more sampling results as extensions of Fig.7 in the main paper. Fig.~\ref{fig:supp_Market_sampling} shows the sampling results (a-e) and real images (f) on Market-1501 dataset.
VAE generates blurry images and DCGAN sharp but unrealistic person images. In contrast, our model generates more realistic images (c)(d)(e). By comparing (d) and (c), we observe that our model using body ROI generates more sharp and realistic images whose colors on each body part are more natural. By comparing (e) and (d), we see that when sampling foreground and background but using the real pose keypoints randomly selected from the training data, we generate better results. 

\begin{figure*} [htp]
\scriptsize
\begin{minipage}{0.33\textwidth}
\centering
  \centering
  \includegraphics[width=0.99\linewidth]{supp_imgs/supp_Market_sampling_a.pdf}\\
(a) Vanilla VAE
\vspace{1mm}
\end{minipage}
\hfill
\begin{minipage}{0.33\textwidth}
\centering
  \centering
  \includegraphics[width=0.99\linewidth]{supp_imgs/supp_Market_sampling_b.pdf}\\
(b) Vanilla DCGAN
\vspace{1mm}
\end{minipage}
\hfill
\begin{minipage}{0.33\textwidth}
\centering
  \centering
  \includegraphics[width=0.99\linewidth]{supp_imgs/supp_Market_sampling_c.pdf}\\
(c) Ours - Whole Body
\vspace{1mm}
\end{minipage}
\hfill
\begin{minipage}{0.33\textwidth}
\centering
  \centering
  \includegraphics[width=0.99\linewidth]{supp_imgs/supp_Market_sampling_d.pdf}\\
(d) Ours - BodyROI7
\end{minipage}
\hfill
\begin{minipage}{0.33\textwidth}
\centering
  \centering
  \includegraphics[width=0.99\linewidth]{supp_imgs/supp_Market_sampling_e.pdf}\\
(e) Ours - BodyROI7 with real pose from training set
\end{minipage}
\hfill
\begin{minipage}{0.33\textwidth}
\centering
  \centering
  \includegraphics[width=0.99\linewidth]{supp_imgs/supp_Market_sampling_f.pdf}\\
(f) Real data
\end{minipage}
\caption{Sampling results. (a) Vanilla VAE; (b) Vanilla DCGAN; (c) Ours - Whole Body; (d) Ours - BodyROI7; (e) Ours - BodyROI7 pose with real pose from training set; (f) Real data. }
\label{fig:supp_Market_sampling}
\end{figure*}

